Preference Poisoning Attacks on Reward Model Learning

Learning reward models from pairwise comparisons is a fundamental component in a number of domains, including autonomous control, conversational agents, and recommendation systems, as part of a broad goal of aligning automated decisions with user preferences. These approaches entail collecting preference information from people, with feedback often provided anonymously. Since preferences are subjective, there is no gold standard to compare against; yet, reliance of high-impact systems on preference learning creates a strong motivation for malicious actors to skew data collected in this fashion to their ends. We investigate the nature and extent of this vulnerability by considering an attacker who can flip a small subset of preference comparisons to either promote or demote a target outcome. We propose two classes of algorithmic approaches for these attacks: a gradient-based framework, and several variants of rank-by-distance methods. Next, we evaluate the efficacy of best attacks in both these classes in successfully achieving malicious goals on datasets from three domains: autonomous control, recommendation system, and textual prompt-response preference learning. We find that the best attacks are often highly successful, achieving in the most extreme case 100\% success rate with only 0.3\% of the data poisoned. However, \emph{which} attack is best can vary significantly across domains. In addition, we observe that the simpler and more scalable rank-by-distance approaches are often competitive with, and on occasion significantly outperform, gradient-based methods. Finally, we show that state-of-the-art defenses against other classes of poisoning attacks exhibit limited efficacy in our setting.

==> test.tex <==
Learning reward models from pairwise comparisons is a fundamental component in a number of domains, including autonomous control, conversational agents, and recommendation systems, as part of a broad goal of aligning automated decisions with user preferences. These approaches entail collecting preference information from people, with feedback often provided anonymously. Since preferences are subjective, there is no gold standard to compare against; yet, reliance of high-impact systems on preference learning creates a strong motivation for malicious actors to skew data collected in this fashion to their ends. We investigate the nature and extent of this vulnerability by considering an attacker who can flip a small subset of preference comparisons to either promote or demote a target outcome. We propose two classes of algorithmic approaches for these attacks: a gradient-based framework, and several variants of rank-by-distance methods. Next, we evaluate the efficacy of best attacks in both these classes in successfully achieving malicious goals on datasets from three domains: autonomous control, recommendation system, and textual prompt-response preference learning. We find that the best attacks are often highly successful, achieving in the most extreme case 100\% success rate with only 0.3\% of the data poisoned. However, \emph{which} attack is best can vary significantly across domains. In addition, we observe that the simpler and more scalable rank-by-distance approaches are often competitive with, and on occasion significantly outperform, gradient-based methods. Finally, we show that state-of-the-art defenses against other classes of poisoning attacks exhibit limited efficacy in our setting.

==> theory.tex <==
\section{Theoretical Guarantee}

\begin{lemma}
Suppose $F$ is a vector space of real-valued functions, and $H = \{\mathbf{1}_{\{f + f(a) \geq 0\}}: f \in F\}$, where $a$ is a constant, then VCdim$(H) \leq \text{dim}(F) + 1 $.%
\label{vcdim}
\end{lemma}
\begin{proof}
    First, we discuss the case where $f_i(a)$ has the same sign for all $i$. 
    Let $\{f_1, f_2, \cdots, f_d\}$ be a basis of $F$. Then if $\{x_1, x_2, \cdots, x_m\}$ is shattered by $H$, there are vectors $v_1, v_2, \cdots, v_{2^m}$ taking all possible sign patterns, and corresponding $w_1, w_2, \cdots, w_{2^m} \in \mathbb{R}^d$ such that $M(w_1 \cdots w_{2^m}) = V - C$, where $M_{i,j} = f_i(x_j)$, $V_{i, j} = v_{i,j}$ and $C_{i,j} = f_i(a)$.
    If $m > d$ then the matrix $M$ is not row-rank $m$. Without loss of generality, we assume the last row can be written as a linear combination of other rows, meaning for some $\alpha_1, \cdots, \alpha_{m - 1}$ we have $v_{mi} = \sum_{j = 1}^{m - 1}\alpha_j v_{ji} + (1 - \sum_{j = 1}^{m - 1} \alpha_j) \cdot f_i(a)$. If $(1 - \sum_{j = 1}^{m - 1} \alpha_j) \cdot f_i(a) \geq 0$, then we choose $i$ such that $\alpha_j v_{ji} \geq 0$ for all $j$, this means $v_{mi} \geq 0$. If $(1 - \sum_{j = 1}^{m - 1} \alpha_j) \cdot f_i(a) \leq 0$, then we choose $i$ such that $\alpha_j v_{ji} \leq 0$ for all $j$, this means $v_{mi} \leq 0$. This contradicts the assumption that $v_i$ together take on all $2^m$ sign patterns. 

    Now we discuss a general case where we do not have the assumption that $f_i(a), \forall i$ has the same sign. Let $\{f_1, f_2, \cdots, f_d\}$ be a basis of $F$. If $1 \in \{f_1, f_2, \cdots, f_d\}$, then $\{1, f_1 - c_1, \cdots, f_d - c_d\}$ is also a basis vector (they are also linearly independent), we can choose $c_1, \cdots, c_d$ such that $f_i(a) - c_i \geq 0$, otherwise, we add $1$ to the basis vectors of $F$. Then we have VCdim$(H) \leq$  dim$(F)$ + 1.
\end{proof}


\begin{theorem}[\citet{anthony1999neural}]
Suppose that \( H \) is a set of functions from a set \( X \) to \( \{0,1\} \) and that \( H \) has finite Vapnik-Chervonenkis dimension \( d \geq 1 \). Let \( L \) be any sample error minimization algorithm for \( H \). Then \( L \) is a learning algorithm for \( H \). In particular, if \( m \geq d/2 \) then %
its sample complexity satisfies the inequality
\[
m_L(\varepsilon, \gamma) \leq m_0(\varepsilon, \gamma) = \frac{64}{\varepsilon^2} \left( 2d \ln \left( \frac{12}{\varepsilon} \right) + \ln \left( \frac{4}{\gamma} \right) \right).
\]
Here $m_L(\varepsilon, \gamma) = \min\{m : m$ is a sufficient sample size for $(\varepsilon, \gamma)$-learning  $H \text{ by } L\},
$ meaning for \( m \geq m_0(\varepsilon, \gamma) \) and $z \in Z^m$ chosen according to $P^m$,
$P^m \{ \text{er}_P(L(z)) < \text{opt}_P(H) + \varepsilon \} \geq 1 - \gamma.$
\label{vc_theorem}
\end{theorem}
\begin{theorem}
    Let  ${\hat{F}(\delta) = \sum_{i=1}^N \mathbf{1}_{\{f(x_T, \theta(\delta)) - f(x_i, \theta(\delta)) \geq 0\}}}$, and $F(\delta) = E_{x\sim P} [\mathbf{1}_{\{f(x_T; \theta(\delta)) - f(x; \theta(\delta)) \geq 0\}}]$, $\delta \in \Delta$.
    Let $F$ be the vector space of real-valued functions with a given structure (e.g., a linear function, or a neural network with ReLU activation function), and $F' = \{f(x; \theta (\delta)) | \theta(\delta) \in \Theta\}$ is the restricted real-valued function space of $F$ induced by $\Delta$. Given dim$(F) = d$, $m_0(\epsilon, \gamma) = \frac{64}{\varepsilon^2} \left( 2(d + 1) \ln \left( \frac{12}{\varepsilon} \right) + \ln \left( \frac{4}{\gamma} \right) \right)$, we have  \[
P^m \{ \max_{\delta \in \Delta} \hat{F}(\delta) < \max_{\delta \in \Delta} {F}(\delta) + \varepsilon \} \geq 1 - \gamma \text{ for } N > m_0(\epsilon, \gamma).\]
\end{theorem}
\begin{proof}
Since $F' \subseteq F$, we have dim$(F')\leq$ dim$(F)$. Let $H = \{\mathbf{1}_{\{f(x_T) - f \geq 0\}} : f \in F'\}$, which is a class of functions that map from a set $X$ to $\{0,1\}$. We set the correct label for all $x \in X$ to be $1$. Let $er_P(h) = P\{(x, y) \in Z: h(x) \neq 1\}$, and $\widehat{er}_z(h) = \frac{1}{N}|\{i: 1 \leq i\leq m \text{ and } h(x_i) \neq 1\}|$, $h \in H$. $opt_P(H) = \inf_{g \in H} er_P(g) = \max_{\delta \in \Delta} F(\delta)$, and $\widehat{er}_z(L(z)) = \min_{h \in H} \widehat{er}_z(h)$. We can then apply Lemma \ref{vcdim} and Theorem  \ref{vc_theorem} to get the results in the theorem.
\end{proof}



        

\section{Counterexample for Heuristic Approach}
Assume there are two data points, $(y_{1,1}, y_{1,2}, o_1 = 0), (y_{2,1}, y_{2,2}, o_2 = 0)$. Let $y_{1,1} - y_{1,2} = [1,0]$, and $y_{2,1} - y_{2,2} = [0,1]$. $|\theta_1| + |\theta_2| = 1$. The optimal $\theta = [0.5, 0.5]$. Let our target candidate be $y_{1,2} = [1,1]$, and $y_{1,1} = [2,1]$. If we flip this label $\theta = [-0.5, 0.5]$, the reward for the target candidate decreases.
